OoDAnalyzer: Interactive Analysis of Out-of-Distribution Samples

One major cause of performance degradation in predictive models is that the test samples are not well covered by the training data. Such not well-represented samples are called OoD samples. In this paper, we propose OoDAnalyzer, a visual analysis approach for interactively identifying OoD samples and explaining them in context. Our approach integrates an ensemble OoD detection method and a grid-based visualization. The detection method is improved from deep ensembles by combining more features with algorithms in the same family. To better analyze and understand the OoD samples in context, we have developed a novel kNN-based grid layout algorithm motivated by Hall's theorem. The algorithm approximates the optimal layout and has $O(kN^2)$ time complexity, faster than the grid layout algorithm with overall best performance but $O(N^3)$ time complexity. Quantitative evaluation and case studies were performed on several datasets to demonstrate the effectiveness and usefulness of OoDAnalyzer.

==> background.tex <==
\section{Background}\label{sec:back}

In this section, we introduce how to generate adversarial examples.

==> conclusion.tex <==
\section{Conclusion}
We have presented a robustness-motivated visual analytics approach that helps experts understand the inner workings of adversarial examples and diagnoses the root cause of incorrect predictions introduced by the adversarial examples. 
The major feature of this approach is that it centers on the concept of datapaths to tightly combine datapath extraction and visualization. 
Two case studies were conducted with two machine learning experts to demonstrate the effectiveness and usefulness of our approach in analyzing both white-box and black-box adversarial examples. 

One interesting avenue for future \doc{research} is to monitor the online testing process, detect potentially adversarial examples, and remove  them from any further processing. 
%work
The key is to design a set of streaming visualizations that can incrementally integrate the \doc{incoming} log data with \doc{existing data}. 
%the existing one new coming
We would also like to continue working with the machine learning experts to conduct several field experiments, \doc{with the aim of} designing  more targeted and effective defense solutions based on the discovered root cause. 
%which aims at 
Another important direction is to analyze the robustness of other types of DNNs, such as RNNs and DGMs. 
For these types of DNNs, exciting research topics include more efficient datapath extraction algorithms and suitable visualizations  for different types of DNNs. 
